A Machine Learning Approach to Recovery of Scene Geometry from Images

Recovering the 3D structure of the scene from images yields useful information for tasks such as shape and scene recognition, object detection, or motion planning and object grasping in robotics. In this thesis, we introduce a general machine learning approach called unsupervised CRF learning based on maximizing the conditional likelihood. We apply our approach to computer vision systems that recover the 3-D scene geometry from images. We focus on recovering 3D geometry from single images, stereo pairs and video sequences. Building these systems requires algorithms for doing inference as well as learning the parameters of conditional Markov random fields (MRF). Our system is trained unsupervisedly without using ground-truth labeled data. We employ a slanted-plane stereo vision model in which we use a fixed over-segmentation to segment the left image into coherent regions called superpixels, then assign a disparity plane for each superpixel. Plane parameters are estimated by solving an MRF labelling problem, through minimizing an energy fuction. We demonstrate the use of our unsupervised CRF learning algorithm for a parameterized slanted-plane stereo vision model involving shape from texture cues. Our stereo model with texture cues, only by unsupervised training, outperforms the results in related work on the same stereo dataset. In this thesis, we also formulate structure and motion estimation as an energy minimization problem, in which the model is an extension of our slanted-plane stereo vision model that also handles surface velocity. Velocity estimation is achieved by solving an MRF labeling problem using Loopy BP. Performance analysis is done using our novel evaluation metrics based on the notion of view prediction error. Experiments on road-driving stereo sequences show encouraging results.

==> contents.tex <==
%
% Contents
%

\tableofcontents

\listoffigures

\listoftables


==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}
We have implemented a prototype compiler for the \mlpolyr{} language
in Standard ML. It retains all of the features that we have
disscussed, including row polymorphism for records and sums,
polymorphic sums, extensible first-class cases as well as type-safe
exception handlers.  The compiler produces machine code for the
PowerPC architecture that can run on Apple Macintosh computers. It
also supports x86 backend based on C-{}-\cite{Jones_cmm}. 

\subsection{Compiler Phases}

The compiler is structured in a fairly traditional way and consists of
the following phases:

\begin{itemize}%\setlength{\itemsep}{0pt}
\item{\bf lexer} lexical analysis, tokenization
\item{\bf parser} LALR(1) parser, generating abstract syntax trees (AST)
\item{\bf elaborator} perform type reconstruction and generation of
  annotated abstract syntax (Absyn)
\item{\bf translate} generate index-passing \lambdarec code
\item{\bf anf-convert} convert \lambdarec code into A-normal
  form~\cite{felleisen93:essence}
\item{\bf anf-optimize} perform various optimization including
  flattening, uncurrying, constant folding, simple constant- and value
  propagation, elimination of useless bindings, short-circuit
  selection from known tuples, inline tiny functions, some arithmetic
  expression simplification
\item{\bf closure} convert to first-order code by closure conversion
\item{\bf clusters} separate closure-converted blocks into clusters of
  blocks; each cluster roughly corresponds to a single C function but
  may have multiple entry points
\item{\bf value-numbering} perform simple common subexpression (CSE) within
  basic blocks
\item{\bf treeify} re-grow larger expression trees to make tree-tiling
  instruction selection more useful
\item{\bf traceschedule} arrange basic blocks to minimize unconditional jumps
\item{\bf cg} perform instruction selection by tree-tiling (maximum-munch algorithm), graph-coloring register allocation; emit assembly code
\end{itemize}

Each phase is implemented in a separate module and a main driver calls
them sequentially as illustrated in \figref{compiler}.

\begin{figure}
\begin{lstlisting}[style=mlpolyr]
(* val main : string * string list -> OS.Process.status *)
fun main (self, args) =
    let val file = Command.parse args
        val ast = Parse.parse file
        val absyn = Elaborate.elaborate ast
        val lambda = Translate.translate absyn
        val anf = LambdaToANF.convert lambda
        val anf_op = Optimize.optimize anf
        val closed = Closure.convert anf
        val {entrylabel, clusters} = Clusters.clusterify closed
        val clusters_cse = ValueNumbering.cse clusters
        val bbt_clusters = Treeify.treeify clusters_cse
        val traces = TraceSchedule.schedule bbt_clusters
        val _ = CodeGen.codegen (traces, entrylabel, file)
    in OS.Process.success
    end
\end{lstlisting}
\caption{A main driver for the \mlpolyr{} compiler.}
\label{fig:compiler}
\end{figure}

\subsection{Runtime system}
The runtime system, written in C, implements a simple two-space
copying garbage collector~\cite{Pierce02} and provides basic
facilities for input and output.

For the tracing garbage collector to be able to reliably distinguish
between pointers and integers, we employ the usual tagging trick.
Integers are 31-bit 2's-complement numbers.  An integer value $i$ is
represented internally as a 2's-complement 32-bit quantity of value
$2i$. This makes all integers even, with their least significant bits
cleared.  Heap pointers, on the other hand, are represented as odd
32-bit values.  In effect, instead of pointing to the beginning of a
word-aligned heap object, they point to the object's second byte.
Generated load- and store-instructions account for this skew by using
an accordingly adjusted displacement value.  With this representation
trick, the most common arithmetic operations (addition and
subtraction) can be implemented as single instructions as usual; they
do not need to manipulate tag bits.  The same is true for most loads
and stores.

\input{fig-strings}

\mlpolyr{} also supports minimal built-in functions as a record value
bound to the global variable {\tt String} as shown in
\figref{string}. This record is allocated using C code and does not
reside within the \mlpolyr{} heap. It contains routines for
manipulating string values, for converting from and to strings, and
for performing simple I/O operations.  Each routine can be accessed by
dot notation. For example, $\mathsf{String.compare}$ could be used to
compare two string values.  Their implementations are hidden inside
the \mlpolyr{} runtime system.



